Self-Aware Adaptive Alignment: Enabling Accurate Perception for Intelligent Transportation Systems

Achieving top-notch performance in Intelligent Transportation detection is a critical research area. However, many challenges still need to be addressed when it comes to detecting in a cross-domain scenario. In this paper, we propose a Self-Aware Adaptive Alignment (SA3), by leveraging an efficient alignment mechanism and recognition strategy. Our proposed method employs a specified attention-based alignment module trained on source and target domain datasets to guide the image-level features alignment process, enabling the local-global adaptive alignment between the source domain and target domain. Features from both domains, whose channel importance is re-weighted, are fed into the region proposal network, which facilitates the acquisition of salient region features. Also, we introduce an instance-to-image level alignment module specific to the target domain to adaptively mitigate the domain gap. To evaluate the proposed method, extensive experiments have been conducted on popular cross-domain object detection benchmarks. Experimental results show that SA3 achieves superior results to the previous state-of-the-art methods.

==> ref0.tex <==

\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
\bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
\bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
\bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
\bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






%%%%no-need%%%%
\bibitem{bbbbbbb9}
M.~Everingham, L.~Van~Gool, C.~K. Williams, J.~Winn, and A.~Zisserman, ``The pascal visual object classes (voc) challenge,'' \emph{International journal of computer vision}, vol.~88, pp. 303--338, 2010.
\bibitem{bbbbbb10}
N.~Inoue, R.~Furuta, T.~Yamasaki, and K.~Aizawa, ``Cross-domain weakly-supervised object detection through progressive domain adaptation,'' in \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, 2018, pp. 5001--5009.
\bibitem{bbbbbbb13}
C.~Chen, J.~Li, Z.~Zheng, Y.~Huang, X.~Ding, and Y.~Yu, ``Dual bipartite graph learning: A general approach for domain adaptive object detection,'' in \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2021, pp. 2703--2712.
\bibitem{bbbbbb24}
M.~Shirpour, N.~Khairdoost, M.~A. Bauer, and S.~S. Beauchemin, ``Traffic object detection and recognition based on the attentional visual field of drivers,'' \emph{IEEE Transactions on Intelligent Vehicles}, vol.~8, no.~1, pp. 594--604, 2021.


\end{thebibliography}

==> test/minipage-fig5.tex <==
\begin{figure*}
	\centering
	\begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-1.png}
		\label{51}
	\end{minipage}
	\begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-2.png}
		\label{52}
	\end{minipage}
        \begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-3.png}
		\label{53}
	\end{minipage}
        \begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-4.png}
		\label{54}  %文中引用该图片代号
	\end{minipage}
	%\qquad
	%让图片换行
	
	\begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-5.png}
		\caption{H2FA}
		\label{55}
	\end{minipage}
	\begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-6.png}
		\caption{SA3 R-CNN}
		\label{56}
	\end{minipage}
        \begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-7.png}
		\caption{H2FA}
		\label{57}
	\end{minipage}
        \begin{minipage}{0.23\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{fig/fig5-8.png}
		\caption{SA3 R-CNN}
		\label{58}%文中引用该图片代号
	\end{minipage}
    
\end{figure*}
